An end-to-end Differentially Private Latent Dirichlet Allocation Using a Spectral Algorithm

We provide an end-to-end differentially private spectral algorithm for learning LDA, based on matrix/tensor decompositions, and establish theoretical guarantees on utility/consistency of the estimated model parameters. The spectral algorithm consists of multiple algorithmic steps, named as "{edges}", to which noise could be injected to obtain differential privacy. We identify \emph{subsets of edges}, named as "{configurations}", such that adding noise to all edges in such a subset guarantees differential privacy of the end-to-end spectral algorithm. We characterize the sensitivity of the edges with respect to the input and thus estimate the amount of noise to be added to each edge for any required privacy level. We then characterize the utility loss for each configuration as a function of injected noise. Overall, by combining the sensitivity and utility characterization, we obtain an end-to-end differentially private spectral algorithm for LDA and identify the corresponding configuration that outperforms others in any specific regime. We are the first to achieve utility guarantees under the required level of differential privacy for learning in LDA. Overall our method systematically outperforms differentially private variational inference.

==> conclusion.tex <==
%!TEX root = 0_nips18_ptm_main.tex
\section{Conclusion}
%
We have provided an end-to-end analysis of differentially private LDA
model using a spectral algorithm.  The algorithm involves a data flow
that permits different locations for injecting noise.

 A fundamental difficulty in this
 problem is that the algorithm involves a complex flow of
 data. Therefore, we provided a detailed sensitivity analysis of
 different parts in this large computational graph. 

Our sensitivity
analysis takes into account the fact that the model consists of $k$
many topics and thereby establishes lower sensitivity bounds once more
data is available. Further, our sensitivity analysis was used to
demonstrate a collection of possible configurations that can achieve
differential privacy. Our analysis, demonstrates that certain
configurations are preferable to others.The analysis that was used can
be extended to other latent variable models where the parameters are
estimated using similar spectral methods such as Gaussian mixtures and
Hidden Markov Models \cite{anandkumar2014tensor}.



==> table_sensitivity.tex <==
%!TEX root = 0_nips18_ptm_main.tex
\begin{table}
\begin{tabular}{l|c|c}
Config. &&\\
(Edge Set) & Constraint & Sensitivity \\
\hline
{\bf 1:} {\small $\widehat{M}_3, \widehat{W}, \widehat{W}^\dag$}& None &
$O(\frac{1}{N})$ \\

($e_3, e_4, e_8$) &&
\\




\hline

{\bf 2:} $\widehat{T},\widehat{W}^\dag$& $\sslda \leq \frac{\sgm{k}-\sgm{k+1}}{2}$ & $O(\frac{k^{3/2}}{N \sigma^{3/2}_k(\slda)})$\\

($e_6, e_8$)&& \\

\hline

{\bf 3:} $\mbar, \widehat{W}^\dag$& $\sslda \leq
\frac{\sgm{k}-\sgm{k+1}}{2}$,  & $O(\frac{k^2}{\ds N \sigma^{3/2}_k(\slda)})$ \\
    
($e_7,e_8$)& $\swt \leq \frac{\ds
  \lambda_k(\wt)}{2\sqrt{k}}$&  \\



%% {\bf 3} $v$ \& $W^\dag$& $e_7$, $e_8$& $\sslda \leq \frac{\sgm{k}-\sgm{k+1}}{2}$ , $\stlda \leq \frac{\ds \lambda_k(\wt)}{2\sqrt{k}}$ & $O(\frac{\sqrt{\sigma_1(\slda)
%%     k^{2.5}}}{\ds N \sk^{3/2}} \tdp{7} + \frac{\sqrt{\sigma_1(\slda)
%%     d}}{\sk N} \tdp{8} $ \\
    
%% &&&  $+\sqrt{\sgm{1}+ \frac{\sqrt{d}}{N} \tdp{8}}
%% \frac{k^{2} \tdp{7}}{\ds N \sgm{1}^{3/2}})$\\

\hline

%{\bf 4} $\mu$ & $e_9$ & $\sslda \leq \frac{\sgm{k}-\sgm{k+1}}{2}$ , $\stlda \leq \frac{\ds \lambda_k(\wt)}{2\sqrt{k}}$  & $O(\frac{\sqrt{\sgm{1}d}k^2}{\ds N \sk^{3/2}} \tdp{9})$\\


{\bf 4:} $\widehat{\mu}$ ($e_9$) & $\sslda \leq \frac{\sgm{k}-\sgm{k+1}}{2}$ ,
 &
$O(\frac{k^2 \sqrt{\sigma_1(\slda)}}{\ds N \sigma^{3/2}_k(\slda)})$\\

 &    $\swt \leq \frac{\ds \lambda_k(\wt)}{2\sqrt{k}}$  &\\



\end{tabular}
\caption{Sensitivity of different configurations that guarantee
  differentially private LDA. The table lists edges in
  Figure~\ref{fig:flow} on which to add Gaussian noise in order to
  achieve differentially private topic model using method of
  moments. $\sslda$ is the sensitivity of $\slda$, $\swt$ is the sensitivity of $\wt$. We use $\tau$ as defined in Proposition~\ref{dp_prop} to decompose the dependence of the noise variance on both the sensitivity and the privacy parameters $\epsilon,\delta$, i.e. $\sigma = \Delta \tdp{i,i}$, where $\Delta$ is the sensitivity. $\widehat{T}
= \tlda(\widehat{W},\widehat{W},\widehat{W})$.} \label{tab:sensitivity}
\end{table}



==> table_symbols.tex <==
%!TEX root = 0_nips18_ptm_main.tex

\newcommand{\symP}[2]{#1~\{#2\}}

\begin{table*}[!htbp]
\begin{tabular}{c|l}
Symbols & Description \\
\hline
{$N$}, {$L$} & Total \# of documents, max. \# of words in a document\\
\symP{$D$}{$D^\prime$} & Document Corpus, Neighboring corpus\\
% & Document Corpus neighboring to $D$\\
%
$l_n$ & Number of words in document $n$\\
\hline
\symP{$\slda$}{$\nslda$}&  Empirical second order LDA moment \{of neighboring corpus\}\\
% & empirical second order LDA moment from neighboring $D^\prime$\\
{ \symP{$\w$}{$\nw$}}& Whitening matrix \{of neighboring corpus\}     \\
%& whitening matrix from neighboring corpus $D^\prime$\\ 
{ \symP{$\wt$}{$\nwt$}} & Whitened tensor \{from neighboring corpus\}\\
$\wtshort$  & Whitened tensor  $\wt$\\
% & whitened tensor resulting from neighboring corpus\\ 
\symP{$\tlda$}{$\ntlda$} & Third order LDA moment \{of neighboring corpus\}\\ 
% & third order LDA moment from neighboring $D^\prime$\\
{\symP{$\sldak$}{$\nsldak$}} & Rank-$k$ approximation of $\slda$ \{of  $\nslda$\} \\
% & rank-$k$ approximation of\\
\hline
$\Delta_{x}$ & Sensitivity of:$\slda$ if $x=2$, $\tlda$ if $x=3$, $\wtshort$ if $x=\wtshort$\\
\hline
$\abar{}$ & Eigenvalue from tensor decomposition \\
$\mbar{}$ & Eigenvector from tensor decomp. before whitening\\
\hline
%% $\swt$ & Sensitivity of whitened tensor \\ 
%% $\svbw$ & sensitivity of vector resulting from the decomposition and before whitening \\
%% $\sabw$ & sensitivity of vector resulting from the decomposition and before whitening\\ 
%% $\sv$ & sensitivity of the output vector (word-topic vector) \\ 
%% $\sa$ & sensitivity of $\alpha_i$ \\
$\ds$ & $min_{i \in [k]} \frac{\sigma_i(\wt)-\sigma_{i+1}(\wt)}{4}$ \\
$\tdp{i}$ & $\frac{\sqrt{2\ln{1.25/\delta_i}}}{\epsilon_i}$  \\
&{\color{red} If you use $\epsilon_i>1$ in the experiment, you need to use this instead: \url{https://github.com/BorjaBalle/analytic-gaussian-mechanism}}
\end{tabular}
\caption{List of Symbols.  Symbols that refer to a neighboring corpus are listed within \{\}. \label{table-symbols}}
\end{table*}


